Measuring and Modeling Neighborhoods

Granular geographic data present new opportunities to understand how neighborhoods are formed, and how they influence politics. At the same time, the inherent subjectivity of neighborhoods creates methodological challenges in measuring and modeling them. We develop an open-source survey instrument that allows respondents to draw their neighborhoods on a map. We also propose a statistical model to analyze how the characteristics of respondents and local areas determine subjective neighborhoods. We conduct two surveys: collecting subjective neighborhoods from voters in Miami, New York City, and Phoenix, and asking New York City residents to draw a community of interest for inclusion in their city council district. Our analysis shows that, holding other factors constant, White respondents include census blocks with more White residents in their neighborhoods. Similarly, Democrats and Republicans are more likely to include co-partisan areas. Furthermore, our model provides more accurate out-of-sample predictions than standard neighborhood measures.

==> header.tex <==
\usepackage{enumerate}
\usepackage{natbib}
\usepackage{hyperref}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{physics}
\usepackage{booktabs}
\usepackage{longtable}
\usepackage{lscape}
\usepackage{subcaption}
\usepackage{setspace}
\usepackage{placeins}

\bibliographystyle{apsr}
\setcitestyle{aysep={}}

\setcounter{secnumdepth}{0}

\captionsetup{font={stretch=1.0}}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\F}{\ensuremath{\mathbb{F}}}
\renewcommand{\empty}{\varnothing}
\newcommand{\f}[1]{\frac{\StrBefore{#1}{/}}{\StrBehind{#1}{/}}} % easier fractions
\newcommand{\half}{\frac{1}{2}}
\newcommand{\eps}{\varepsilon}
\newcommand{\dfeq}{\coloneqq}
\DeclareMathOperator{\E}{\mathbb{E}}
\let\Pr\undefined
\DeclareMathOperator{\Pr}{\mathbb{P}}
\newcommand{\indep}{\mathbin{\perp\!\!\!\!\!\:\perp}}
\newcommand{\gvn}{\;\middle|\;}
\renewcommand{\F}{\ensuremath{\mathcal{F}}}
\newcommand{\B}{\ensuremath{\mathcal{B}}}
\newcommand{\ind}{\mathbf{1}}
\DeclareMathOperator{\Var}{\mathbb{V}}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Corr}{Corr}
\DeclareMathOperator{\Unif}{Unif}
\newcommand{\Bernoulli}{\mathrm{Bernoulli}\qty}
\newcommand{\Norm}{\mathcal{N}\qty}
\newcommand{\MVNorm}[1][]{\mathcal{N}_{#1}\qty}
\DeclareMathOperator{\Student}{Student-\mathit{t}}
\DeclarePairedDelimiter\br{\langle}{\rangle}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclarePairedDelimiter\round{\lceil}{\rfloor}


==> tables/city-pop-summary.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Sun Oct  8 10:32:07 2023
\begin{table}[ht]
\centering
\begin{tabular}{rlll}
  \hline
 & 1 & 2 & 3 \\ 
  \hline
city & miami & new-york & phoenix \\ 
  pct\_college & 0.413 & 0.455 & 0.389 \\ 
  pct\_homeown & 0.608 & 0.449 & 0.641 \\ 
  med\_inc & 66944 & 85267 & 71421 \\ 
  pct\_reg & 0.650 & 0.614 & 0.656 \\ 
  pct\_white & 0.348 & 0.420 & 0.587 \\ 
  pct\_black & 0.197 & 0.181 & 0.046 \\ 
  pct\_hisp & 0.416 & 0.263 & 0.295 \\ 
  pct\_dem & 0.450 & 0.587 & 0.313 \\ 
  pct\_rep & 0.247 & 0.148 & 0.343 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/model_coef_full_housing.tex <==
\begingroup\fontsize{10}{12}\selectfont

\begin{longtable}[t]{llrrrrr}
\caption{Full model estimates.}\\
\toprule
Coefficient & City & Mean & Std. Dev. & Q5 & Median & Q95\\
\midrule
\cellcolor{gray!6}{(Intercept)} & \cellcolor{gray!6}{Miami} & \cellcolor{gray!6}{-9.00} & \cellcolor{gray!6}{10.68} & \cellcolor{gray!6}{-25.81} & \cellcolor{gray!6}{-9.03} & \cellcolor{gray!6}{8.70}\\
\cellcolor{gray!6}{(Intercept)} & \cellcolor{gray!6}{NYC} & \cellcolor{gray!6}{-6.73} & \cellcolor{gray!6}{6.42} & \cellcolor{gray!6}{-17.83} & \cellcolor{gray!6}{-6.64} & \cellcolor{gray!6}{3.52}\\
\cellcolor{gray!6}{(Intercept)} & \cellcolor{gray!6}{Phoenix} & \cellcolor{gray!6}{-8.98} & \cellcolor{gray!6}{6.15} & \cellcolor{gray!6}{-18.71} & \cellcolor{gray!6}{-8.80} & \cellcolor{gray!6}{1.14}\\
Church & Miami & 0.02 & 0.07 & -0.09 & 0.02 & 0.12\\
Church & NYC & 0.14 & 0.04 & 0.08 & 0.14 & 0.21\\
Church & Phoenix & 0.18 & 0.04 & 0.11 & 0.18 & 0.25\\
\cellcolor{gray!6}{Distance} & \cellcolor{gray!6}{Miami} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{0.02} & \cellcolor{gray!6}{0.00} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{0.07}\\
\cellcolor{gray!6}{Distance} & \cellcolor{gray!6}{Miami} & \cellcolor{gray!6}{0.20} & \cellcolor{gray!6}{0.03} & \cellcolor{gray!6}{0.15} & \cellcolor{gray!6}{0.20} & \cellcolor{gray!6}{0.26}\\
\cellcolor{gray!6}{Distance} & \cellcolor{gray!6}{NYC} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{0.02} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{0.16}\\
Distance & NYC & -0.04 & 0.03 & -0.08 & -0.04 & 0.00\\
Distance & Phoenix & 0.10 & 0.01 & 0.08 & 0.10 & 0.12\\
Distance & Phoenix & 0.17 & 0.02 & 0.14 & 0.16 & 0.19\\
\cellcolor{gray!6}{Park} & \cellcolor{gray!6}{Miami} & \cellcolor{gray!6}{-0.17} & \cellcolor{gray!6}{0.09} & \cellcolor{gray!6}{-0.33} & \cellcolor{gray!6}{-0.17} & \cellcolor{gray!6}{-0.03}\\
\cellcolor{gray!6}{Park} & \cellcolor{gray!6}{NYC} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{0.07} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{0.19}\\
\cellcolor{gray!6}{Park} & \cellcolor{gray!6}{Phoenix} & \cellcolor{gray!6}{0.12} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{0.06} & \cellcolor{gray!6}{0.12} & \cellcolor{gray!6}{0.19}\\
School & Miami & 0.49 & 0.15 & 0.24 & 0.49 & 0.75\\
School & NYC & -0.18 & 0.11 & -0.36 & -0.18 & 0.00\\
School & Phoenix & 0.21 & 0.07 & 0.10 & 0.21 & 0.33\\
\cellcolor{gray!6}{Children} & \cellcolor{gray!6}{Miami} & \cellcolor{gray!6}{1.68} & \cellcolor{gray!6}{3.48} & \cellcolor{gray!6}{-3.99} & \cellcolor{gray!6}{1.69} & \cellcolor{gray!6}{7.51}\\
\cellcolor{gray!6}{Children} & \cellcolor{gray!6}{NYC} & \cellcolor{gray!6}{-0.84} & \cellcolor{gray!6}{2.30} & \cellcolor{gray!6}{-4.69} & \cellcolor{gray!6}{-0.86} & \cellcolor{gray!6}{2.89}\\
\cellcolor{gray!6}{Children} & \cellcolor{gray!6}{Phoenix} & \cellcolor{gray!6}{-0.84} & \cellcolor{gray!6}{2.06} & \cellcolor{gray!6}{-4.33} & \cellcolor{gray!6}{-0.88} & \cellcolor{gray!6}{2.57}\\
Same block group & Miami & 0.08 & 0.07 & -0.03 & 0.08 & 0.20\\
Same block group & NYC & 0.38 & 0.08 & 0.25 & 0.38 & 0.50\\
Same block group & Phoenix & 0.05 & 0.03 & 0.00 & 0.05 & 0.10\\
\cellcolor{gray!6}{Same tract} & \cellcolor{gray!6}{Miami} & \cellcolor{gray!6}{-0.45} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{-0.62} & \cellcolor{gray!6}{-0.45} & \cellcolor{gray!6}{-0.27}\\
\cellcolor{gray!6}{Same tract} & \cellcolor{gray!6}{NYC} & \cellcolor{gray!6}{0.21} & \cellcolor{gray!6}{0.09} & \cellcolor{gray!6}{0.06} & \cellcolor{gray!6}{0.21} & \cellcolor{gray!6}{0.35}\\
\cellcolor{gray!6}{Same tract} & \cellcolor{gray!6}{Phoenix} & \cellcolor{gray!6}{-0.01} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{-0.17} & \cellcolor{gray!6}{-0.01} & \cellcolor{gray!6}{0.15}\\
Same road region & Miami & -0.56 & 0.05 & -0.64 & -0.56 & -0.48\\
Same road region & NYC & 0.08 & 0.03 & 0.02 & 0.08 & 0.14\\
Same road region & Phoenix & -0.06 & 0.03 & -0.10 & -0.06 & -0.01\\
\cellcolor{gray!6}{Population} & \cellcolor{gray!6}{Miami} & \cellcolor{gray!6}{-0.40} & \cellcolor{gray!6}{0.26} & \cellcolor{gray!6}{-0.83} & \cellcolor{gray!6}{-0.40} & \cellcolor{gray!6}{0.04}\\
\cellcolor{gray!6}{Population} & \cellcolor{gray!6}{NYC} & \cellcolor{gray!6}{-0.98} & \cellcolor{gray!6}{0.17} & \cellcolor{gray!6}{-1.25} & \cellcolor{gray!6}{-0.99} & \cellcolor{gray!6}{-0.72}\\
\cellcolor{gray!6}{Population} & \cellcolor{gray!6}{Phoenix} & \cellcolor{gray!6}{-1.21} & \cellcolor{gray!6}{0.16} & \cellcolor{gray!6}{-1.48} & \cellcolor{gray!6}{-1.20} & \cellcolor{gray!6}{-0.95}\\
Area & Miami & -0.36 & 0.09 & -0.51 & -0.36 & -0.21\\
Area & NYC & -0.04 & 0.07 & -0.16 & -0.04 & 0.08\\
Area & Phoenix & -0.06 & 0.04 & -0.12 & -0.06 & 0.00\\
\cellcolor{gray!6}{Fraction same race} & \cellcolor{gray!6}{Miami} & \cellcolor{gray!6}{-0.19} & \cellcolor{gray!6}{0.12} & \cellcolor{gray!6}{-0.38} & \cellcolor{gray!6}{-0.18} & \cellcolor{gray!6}{0.00}\\
\cellcolor{gray!6}{Fraction same race} & \cellcolor{gray!6}{NYC} & \cellcolor{gray!6}{-0.15} & \cellcolor{gray!6}{0.09} & \cellcolor{gray!6}{-0.29} & \cellcolor{gray!6}{-0.15} & \cellcolor{gray!6}{0.00}\\
\cellcolor{gray!6}{Fraction same race} & \cellcolor{gray!6}{Phoenix} & \cellcolor{gray!6}{-0.57} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{-0.72} & \cellcolor{gray!6}{-0.57} & \cellcolor{gray!6}{-0.40}\\
Housing & Miami & 1.02 & 10.16 & -14.93 & 1.04 & 17.58\\
Housing & NYC & 0.16 & 4.26 & -6.77 & 0.02 & 7.19\\
Housing & Phoenix & -0.38 & 7.11 & -11.74 & -0.24 & 11.20\\
\cellcolor{gray!6}{Homeowner} & \cellcolor{gray!6}{Miami} & \cellcolor{gray!6}{0.29} & \cellcolor{gray!6}{5.69} & \cellcolor{gray!6}{-9.48} & \cellcolor{gray!6}{0.51} & \cellcolor{gray!6}{9.54}\\
\cellcolor{gray!6}{Homeowner} & \cellcolor{gray!6}{NYC} & \cellcolor{gray!6}{-0.20} & \cellcolor{gray!6}{2.77} & \cellcolor{gray!6}{-4.69} & \cellcolor{gray!6}{-0.40} & \cellcolor{gray!6}{4.37}\\
\cellcolor{gray!6}{Homeowner} & \cellcolor{gray!6}{Phoenix} & \cellcolor{gray!6}{-0.37} & \cellcolor{gray!6}{4.01} & \cellcolor{gray!6}{-7.04} & \cellcolor{gray!6}{-0.25} & \cellcolor{gray!6}{6.00}\\
Fraction same party & Miami & -0.31 & 0.09 & -0.45 & -0.31 & -0.17\\
Fraction same party & NYC & -0.29 & 0.07 & -0.40 & -0.29 & -0.17\\
Fraction same party & Phoenix & -0.27 & 0.05 & -0.36 & -0.27 & -0.18\\
\cellcolor{gray!6}{Fraction same ownership} & \cellcolor{gray!6}{Miami} & \cellcolor{gray!6}{-0.29} & \cellcolor{gray!6}{0.15} & \cellcolor{gray!6}{-0.53} & \cellcolor{gray!6}{-0.29} & \cellcolor{gray!6}{-0.04}\\
\cellcolor{gray!6}{Fraction same ownership} & \cellcolor{gray!6}{NYC} & \cellcolor{gray!6}{-0.18} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{-0.36} & \cellcolor{gray!6}{-0.18} & \cellcolor{gray!6}{0.01}\\
\cellcolor{gray!6}{Fraction same ownership} & \cellcolor{gray!6}{Phoenix} & \cellcolor{gray!6}{-0.30} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{-0.47} & \cellcolor{gray!6}{-0.29} & \cellcolor{gray!6}{-0.12}\\
Fraction same education & Miami & -0.16 & 0.13 & -0.36 & -0.17 & 0.04\\
Fraction same education & NYC & -0.62 & 0.07 & -0.73 & -0.62 & -0.49\\
Fraction same education & Phoenix & -0.89 & 0.06 & -1.00 & -0.89 & -0.79\\
\cellcolor{gray!6}{Age} & \cellcolor{gray!6}{Miami} & \cellcolor{gray!6}{0.01} & \cellcolor{gray!6}{0.19} & \cellcolor{gray!6}{-0.29} & \cellcolor{gray!6}{0.01} & \cellcolor{gray!6}{0.33}\\
\cellcolor{gray!6}{Age} & \cellcolor{gray!6}{NYC} & \cellcolor{gray!6}{0.01} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{-0.16} & \cellcolor{gray!6}{0.01} & \cellcolor{gray!6}{0.17}\\
\cellcolor{gray!6}{Age} & \cellcolor{gray!6}{Phoenix} & \cellcolor{gray!6}{0.01} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{-0.18} & \cellcolor{gray!6}{0.01} & \cellcolor{gray!6}{0.18}\\
Education = no college & Miami & -0.56 & 3.36 & -5.84 & -0.47 & 5.00\\
Education = no college & NYC & -1.21 & 2.46 & -5.09 & -1.11 & 2.81\\
Education = no college & Phoenix & 0.10 & 2.02 & -3.22 & -0.05 & 3.46\\
\cellcolor{gray!6}{Retired} & \cellcolor{gray!6}{Miami} & \cellcolor{gray!6}{0.38} & \cellcolor{gray!6}{3.47} & \cellcolor{gray!6}{-5.25} & \cellcolor{gray!6}{0.39} & \cellcolor{gray!6}{5.98}\\
\cellcolor{gray!6}{Retired} & \cellcolor{gray!6}{NYC} & \cellcolor{gray!6}{0.56} & \cellcolor{gray!6}{2.62} & \cellcolor{gray!6}{-3.49} & \cellcolor{gray!6}{0.43} & \cellcolor{gray!6}{5.17}\\
\cellcolor{gray!6}{Retired} & \cellcolor{gray!6}{Phoenix} & \cellcolor{gray!6}{-0.06} & \cellcolor{gray!6}{2.57} & \cellcolor{gray!6}{-4.10} & \cellcolor{gray!6}{-0.11} & \cellcolor{gray!6}{4.22}\\
Tenure & Miami & -0.12 & 1.03 & -1.91 & -0.13 & 1.52\\
Tenure & NYC & -0.10 & 0.80 & -1.40 & -0.06 & 1.17\\
Tenure & Phoenix & 0.15 & 0.74 & -1.12 & 0.16 & 1.33\\
\cellcolor{gray!6}{Party = ind} & \cellcolor{gray!6}{Miami} & \cellcolor{gray!6}{-0.22} & \cellcolor{gray!6}{4.92} & \cellcolor{gray!6}{-8.14} & \cellcolor{gray!6}{-0.20} & \cellcolor{gray!6}{7.81}\\
\cellcolor{gray!6}{Party = ind} & \cellcolor{gray!6}{NYC} & \cellcolor{gray!6}{0.05} & \cellcolor{gray!6}{3.66} & \cellcolor{gray!6}{-5.90} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{6.30}\\
\cellcolor{gray!6}{Party = ind} & \cellcolor{gray!6}{Phoenix} & \cellcolor{gray!6}{0.09} & \cellcolor{gray!6}{3.39} & \cellcolor{gray!6}{-5.43} & \cellcolor{gray!6}{0.02} & \cellcolor{gray!6}{5.59}\\
Party = rep & Miami & -0.08 & 2.85 & -4.65 & -0.03 & 4.62\\
Party = rep & NYC & -0.29 & 2.18 & -3.94 & -0.27 & 3.28\\
Party = rep & Phoenix & 0.00 & 1.84 & -3.05 & -0.04 & 3.10\\
\cellcolor{gray!6}{Minority} & \cellcolor{gray!6}{Miami} & \cellcolor{gray!6}{-0.37} & \cellcolor{gray!6}{3.93} & \cellcolor{gray!6}{-6.95} & \cellcolor{gray!6}{-0.24} & \cellcolor{gray!6}{5.84}\\
\cellcolor{gray!6}{Minority} & \cellcolor{gray!6}{NYC} & \cellcolor{gray!6}{0.12} & \cellcolor{gray!6}{2.31} & \cellcolor{gray!6}{-3.53} & \cellcolor{gray!6}{0.20} & \cellcolor{gray!6}{3.79}\\
\cellcolor{gray!6}{Minority} & \cellcolor{gray!6}{Phoenix} & \cellcolor{gray!6}{-0.12} & \cellcolor{gray!6}{2.62} & \cellcolor{gray!6}{-4.49} & \cellcolor{gray!6}{-0.11} & \cellcolor{gray!6}{4.17}\\
School * children & Miami & -0.61 & 0.24 & -1.01 & -0.61 & -0.22\\
School * children & NYC & 0.33 & 0.15 & 0.09 & 0.34 & 0.57\\
School * children & Phoenix & 0.19 & 0.11 & -0.01 & 0.18 & 0.37\\
\cellcolor{gray!6}{Children * distance} & \cellcolor{gray!6}{Miami} & \cellcolor{gray!6}{-0.16} & \cellcolor{gray!6}{0.05} & \cellcolor{gray!6}{-0.24} & \cellcolor{gray!6}{-0.16} & \cellcolor{gray!6}{-0.07}\\
\cellcolor{gray!6}{Children * distance} & \cellcolor{gray!6}{NYC} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{0.05} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{0.16}\\
\cellcolor{gray!6}{Children * distance} & \cellcolor{gray!6}{Phoenix} & \cellcolor{gray!6}{0.12} & \cellcolor{gray!6}{0.03} & \cellcolor{gray!6}{0.08} & \cellcolor{gray!6}{0.12} & \cellcolor{gray!6}{0.17}\\
Same tract * same road region & Miami & 0.28 & 0.11 & 0.10 & 0.28 & 0.46\\
Same tract * same road region & NYC & -0.39 & 0.10 & -0.56 & -0.39 & -0.23\\
Same tract * same road region & Phoenix & -0.50 & 0.10 & -0.67 & -0.50 & -0.34\\
\cellcolor{gray!6}{Fraction same race * housing} & \cellcolor{gray!6}{Miami} & \cellcolor{gray!6}{-0.09} & \cellcolor{gray!6}{0.26} & \cellcolor{gray!6}{-0.51} & \cellcolor{gray!6}{-0.10} & \cellcolor{gray!6}{0.37}\\
\cellcolor{gray!6}{Fraction same race * housing} & \cellcolor{gray!6}{NYC} & \cellcolor{gray!6}{0.20} & \cellcolor{gray!6}{0.16} & \cellcolor{gray!6}{-0.06} & \cellcolor{gray!6}{0.20} & \cellcolor{gray!6}{0.45}\\
\cellcolor{gray!6}{Fraction same race * housing} & \cellcolor{gray!6}{Phoenix} & \cellcolor{gray!6}{0.72} & \cellcolor{gray!6}{0.15} & \cellcolor{gray!6}{0.48} & \cellcolor{gray!6}{0.72} & \cellcolor{gray!6}{0.97}\\
Fraction same race * homeowner & Miami & -0.23 & 0.13 & -0.44 & -0.23 & -0.01\\
Fraction same race * homeowner & NYC & -0.03 & 0.10 & -0.20 & -0.04 & 0.13\\
Fraction same race * homeowner & Phoenix & 0.16 & 0.10 & 0.00 & 0.16 & 0.32\\
\cellcolor{gray!6}{Housing * homeowner} & \cellcolor{gray!6}{Miami} & \cellcolor{gray!6}{-1.16} & \cellcolor{gray!6}{10.24} & \cellcolor{gray!6}{-17.71} & \cellcolor{gray!6}{-1.26} & \cellcolor{gray!6}{15.69}\\
\cellcolor{gray!6}{Housing * homeowner} & \cellcolor{gray!6}{NYC} & \cellcolor{gray!6}{-0.44} & \cellcolor{gray!6}{4.87} & \cellcolor{gray!6}{-8.06} & \cellcolor{gray!6}{-0.28} & \cellcolor{gray!6}{7.55}\\
\cellcolor{gray!6}{Housing * homeowner} & \cellcolor{gray!6}{Phoenix} & \cellcolor{gray!6}{0.76} & \cellcolor{gray!6}{7.34} & \cellcolor{gray!6}{-11.16} & \cellcolor{gray!6}{0.50} & \cellcolor{gray!6}{12.62}\\
Housing * fraction same party & Miami & 0.00 & 0.14 & -0.22 & 0.00 & 0.23\\
Housing * fraction same party & NYC & -0.03 & 0.10 & -0.20 & -0.04 & 0.15\\
Housing * fraction same party & Phoenix & 0.10 & 0.08 & -0.04 & 0.09 & 0.24\\
\cellcolor{gray!6}{Homeowner * fraction same ownership} & \cellcolor{gray!6}{Miami} & \cellcolor{gray!6}{0.53} & \cellcolor{gray!6}{0.17} & \cellcolor{gray!6}{0.25} & \cellcolor{gray!6}{0.52} & \cellcolor{gray!6}{0.81}\\
\cellcolor{gray!6}{Homeowner * fraction same ownership} & \cellcolor{gray!6}{NYC} & \cellcolor{gray!6}{0.28} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{0.06} & \cellcolor{gray!6}{0.28} & \cellcolor{gray!6}{0.49}\\
\cellcolor{gray!6}{Homeowner * fraction same ownership} & \cellcolor{gray!6}{Phoenix} & \cellcolor{gray!6}{0.40} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{0.21} & \cellcolor{gray!6}{0.40} & \cellcolor{gray!6}{0.59}\\
Fraction same education * educ = no college & Miami & 0.86 & 0.22 & 0.51 & 0.87 & 1.21\\
Fraction same education * educ = no college & NYC & 1.68 & 0.16 & 1.43 & 1.68 & 1.94\\
Fraction same education * educ = no college & Phoenix & 0.59 & 0.17 & 0.31 & 0.59 & 0.87\\
\cellcolor{gray!6}{Fraction same race * housing * homeowner} & \cellcolor{gray!6}{Miami} & \cellcolor{gray!6}{0.26} & \cellcolor{gray!6}{0.28} & \cellcolor{gray!6}{-0.23} & \cellcolor{gray!6}{0.27} & \cellcolor{gray!6}{0.69}\\
\cellcolor{gray!6}{Fraction same race * housing * homeowner} & \cellcolor{gray!6}{NYC} & \cellcolor{gray!6}{-0.12} & \cellcolor{gray!6}{0.17} & \cellcolor{gray!6}{-0.40} & \cellcolor{gray!6}{-0.12} & \cellcolor{gray!6}{0.16}\\
\cellcolor{gray!6}{Fraction same race * housing * homeowner} & \cellcolor{gray!6}{Phoenix} & \cellcolor{gray!6}{-0.59} & \cellcolor{gray!6}{0.15} & \cellcolor{gray!6}{-0.85} & \cellcolor{gray!6}{-0.59} & \cellcolor{gray!6}{-0.36}\\
Alpha & Miami & 1.28 & 0.04 & 1.21 & 1.28 & 1.35\\
Alpha & NYC & 1.57 & 0.04 & 1.50 & 1.57 & 1.64\\
Alpha & Phoenix & 1.38 & 0.03 & 1.33 & 1.37 & 1.42\\
\bottomrule
\end{longtable}
\endgroup{}

==> tables/nbh-summary-full-nycc.tex <==
\begin{table}
\centering
\begin{tabular}[t]{lrrrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{4}{c}{email} & \multicolumn{4}{c}{meta} & \multicolumn{4}{c}{ } \\
\cmidrule(l{3pt}r{3pt}){2-5} \cmidrule(l{3pt}r{3pt}){6-9}
  & Mean & Median & Min & Max & Mean & Median & Min & Max & Mean & Median & Min & Max\\
\midrule
pop & \num{54025.52} & \num{37680.66} & \num{319.00} & \num{455384.62} & \num{52668.45} & \num{38773.00} & \num{534.39} & \num{210201.47} & \num{53296.12} & \num{38070.00} & \num{319.00} & \num{455384.62}\\
sq.miles & \num{1.06} & \num{0.65} & \num{0.01} & \num{12.41} & \num{0.91} & \num{0.60} & \num{0.03} & \num{5.15} & \num{0.98} & \num{0.63} & \num{0.01} & \num{12.41}\\
dem\_p & \num{0.67} & \num{0.69} & \num{0.21} & \num{0.87} & \num{0.69} & \num{0.70} & \num{0.25} & \num{0.83} & \num{0.68} & \num{0.69} & \num{0.21} & \num{0.87}\\
rep\_p & \num{0.10} & \num{0.08} & \num{0.02} & \num{0.52} & \num{0.09} & \num{0.08} & \num{0.02} & \num{0.47} & \num{0.10} & \num{0.08} & \num{0.02} & \num{0.52}\\
white\_p & \num{0.48} & \num{0.56} & \num{0.00} & \num{0.89} & \num{0.49} & \num{0.56} & \num{0.01} & \num{0.98} & \num{0.49} & \num{0.56} & \num{0.00} & \num{0.98}\\
black\_p & \num{0.16} & \num{0.05} & \num{0.00} & \num{0.92} & \num{0.14} & \num{0.05} & \num{0.00} & \num{0.83} & \num{0.15} & \num{0.05} & \num{0.00} & \num{0.92}\\
\bottomrule
\end{tabular}
\end{table}

==> tables/nbh-summary-full.tex <==
\begin{table}
\centering
\begin{tabular}[t]{lrrrrrrrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{4}{c}{miami} & \multicolumn{4}{c}{new-york} & \multicolumn{4}{c}{phoenix} & \multicolumn{4}{c}{ } \\
\cmidrule(l{3pt}r{3pt}){2-5} \cmidrule(l{3pt}r{3pt}){6-9} \cmidrule(l{3pt}r{3pt}){10-13}
  & Mean & Median & Min & Max & Mean & Median & Min & Max & Mean & Median & Min & Max & Mean & Median & Min & Max\\
\midrule
pop & \num{11921.35} & \num{3175.50} & \num{0.00} & \num{303936.00} & \num{33570.36} & \num{15232.00} & \num{48.00} & \num{344789.00} & \num{8822.97} & \num{2134.00} & \num{0.00} & \num{284947.00} & \num{13840.46} & \num{3020.00} & \num{0.00} & \num{344789.00}\\
sq.miles & \num{3.64} & \num{0.83} & \num{0.01} & \num{125.44} & \num{1.97} & \num{0.69} & \num{0.01} & \num{95.02} & \num{3.95} & \num{0.81} & \num{0.00} & \num{344.74} & \num{3.54} & \num{0.78} & \num{0.00} & \num{344.74}\\
dem\_p & \num{0.41} & \num{0.40} & \num{0.17} & \num{0.82} & \num{0.54} & \num{0.55} & \num{0.11} & \num{0.83} & \num{0.30} & \num{0.28} & \num{0.07} & \num{0.64} & \num{0.36} & \num{0.32} & \num{0.07} & \num{0.83}\\
rep\_p & \num{0.28} & \num{0.28} & \num{0.03} & \num{0.64} & \num{0.18} & \num{0.15} & \num{0.02} & \num{0.52} & \num{0.38} & \num{0.39} & \num{0.06} & \num{0.70} & \num{0.33} & \num{0.34} & \num{0.02} & \num{0.70}\\
white\_p & \num{0.54} & \num{0.58} & \num{0.01} & \num{0.99} & \num{0.62} & \num{0.70} & \num{0.01} & \num{1.00} & \num{0.73} & \num{0.76} & \num{0.02} & \num{1.00} & \num{0.67} & \num{0.73} & \num{0.01} & \num{1.00}\\
black\_p & \num{0.11} & \num{0.06} & \num{0.00} & \num{0.96} & \num{0.10} & \num{0.03} & \num{0.00} & \num{0.83} & \num{0.03} & \num{0.03} & \num{0.00} & \num{0.30} & \num{0.06} & \num{0.03} & \num{0.00} & \num{0.96}\\
\bottomrule
\end{tabular}
\end{table}

==> tables/nbh-summary-party-full-nycc.tex <==
\begin{table}
\centering
\begin{tabular}[t]{lrrrrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{email} & \multicolumn{3}{c}{meta} & \multicolumn{3}{c}{ } \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7}
  & Democrat & Independent & Republican & Democrat & Independent & Republican & Democrat & Independent & Republican\\
\midrule
dem\_p & \num{0.69} & \num{0.67} & \num{0.59} & \num{0.70} & \num{0.71} & \num{0.62} & \num{0.70} & \num{0.69} & \num{0.60}\\
rep\_p & \num{0.09} & \num{0.10} & \num{0.15} & \num{0.08} & \num{0.08} & \num{0.14} & \num{0.09} & \num{0.09} & \num{0.15}\\
\bottomrule
\end{tabular}
\end{table}

==> tables/nbh-summary-party-full.tex <==
\begin{table}
\centering
\begin{tabular}[t]{lrrrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{miami} & \multicolumn{3}{c}{new-york} & \multicolumn{3}{c}{phoenix} & \multicolumn{3}{c}{ } \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7} \cmidrule(l{3pt}r{3pt}){8-10}
  & Democrat & Independent & Republican & Democrat & Independent & Republican & Democrat & Independent & Republican & Democrat & Independent & Republican\\
\midrule
dem\_p & \num{0.42} & \num{0.41} & \num{0.39} & \num{0.58} & \num{0.45} & \num{0.47} & \num{0.31} & \num{0.30} & \num{0.28} & \num{0.40} & \num{0.35} & \num{0.32}\\
rep\_p & \num{0.27} & \num{0.26} & \num{0.31} & \num{0.15} & \num{0.21} & \num{0.22} & \num{0.36} & \num{0.38} & \num{0.40} & \num{0.29} & \num{0.33} & \num{0.36}\\
\bottomrule
\end{tabular}
\end{table}

==> tables/nbh-summary-party-party-nycc.tex <==
\begin{table}
\centering
\begin{tabular}[t]{lrrrrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{email} & \multicolumn{3}{c}{meta} & \multicolumn{3}{c}{ } \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7}
  & Democrat & Independent & Republican & Democrat & Independent & Republican & Democrat & Independent & Republican\\
\midrule
dem\_p & \num{0.69} & \num{0.67} & \num{0.59} & \num{0.70} & \num{0.71} & \num{0.62} & \num{0.70} & \num{0.69} & \num{0.60}\\
rep\_p & \num{0.09} & \num{0.10} & \num{0.15} & \num{0.08} & \num{0.08} & \num{0.14} & \num{0.09} & \num{0.09} & \num{0.15}\\
\bottomrule
\end{tabular}
\end{table}

==> tables/nbh-summary-party.tex <==
\begin{table}
\centering
\begin{tabular}[t]{lrrrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{miami} & \multicolumn{3}{c}{new-york} & \multicolumn{3}{c}{phoenix} & \multicolumn{3}{c}{ } \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7} \cmidrule(l{3pt}r{3pt}){8-10}
\multicolumn{1}{c}{ } & \multicolumn{1}{c}{Democrat} & \multicolumn{1}{c}{Independent} & \multicolumn{1}{c}{Republican} & \multicolumn{1}{c}{Democrat} & \multicolumn{1}{c}{Independent} & \multicolumn{1}{c}{Republican} & \multicolumn{1}{c}{Democrat} & \multicolumn{1}{c}{Independent} & \multicolumn{1}{c}{Republican} & \multicolumn{1}{c}{Democrat} & \multicolumn{1}{c}{Independent} & \multicolumn{1}{c}{Republican} \\
\cmidrule(l{3pt}r{3pt}){2-2} \cmidrule(l{3pt}r{3pt}){3-3} \cmidrule(l{3pt}r{3pt}){4-4} \cmidrule(l{3pt}r{3pt}){5-5} \cmidrule(l{3pt}r{3pt}){6-6} \cmidrule(l{3pt}r{3pt}){7-7} \cmidrule(l{3pt}r{3pt}){8-8} \cmidrule(l{3pt}r{3pt}){9-9} \cmidrule(l{3pt}r{3pt}){10-10} \cmidrule(l{3pt}r{3pt}){11-11} \cmidrule(l{3pt}r{3pt}){12-12} \cmidrule(l{3pt}r{3pt}){13-13}
  & Mean & Mean  & Mean   & Mean    & Mean     & Mean      & Mean       & Mean        & Mean         & Mean          & Mean           & Mean           \\
\midrule
dem\_p & \num{0.43} & \num{0.43} & \num{0.41} & \num{0.57} & \num{0.45} & \num{0.45} & \num{0.30} & \num{0.33} & \num{0.28} & \num{0.38} & \num{0.37} & \num{0.32}\\
rep\_p & \num{0.28} & \num{0.25} & \num{0.28} & \num{0.17} & \num{0.22} & \num{0.23} & \num{0.38} & \num{0.34} & \num{0.40} & \num{0.31} & \num{0.30} & \num{0.36}\\
\bottomrule
\end{tabular}
\end{table}

==> tables/nbh-summary-race-full-nycc.tex <==
\begin{table}
\centering
\begin{tabular}[t]{lrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{email} & \multicolumn{2}{c}{meta} & \multicolumn{2}{c}{ } \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5}
  & non-white & white & non-white & white & non-white & white\\
\midrule
white\_p & \num{0.33} & \num{0.55} & \num{0.37} & \num{0.52} & \num{0.35} & \num{0.53}\\
black\_p & \num{0.26} & \num{0.11} & \num{0.25} & \num{0.11} & \num{0.25} & \num{0.11}\\
\bottomrule
\end{tabular}
\end{table}

==> tables/nbh-summary-race-full.tex <==
\begin{table}
\centering
\begin{tabular}[t]{lrrrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{miami} & \multicolumn{2}{c}{new-york} & \multicolumn{2}{c}{phoenix} & \multicolumn{2}{c}{ } \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7}
  & non-white & white & non-white & white & non-white & white & non-white & white\\
\midrule
white\_p & \num{0.35} & \num{0.62} & \num{0.44} & \num{0.68} & \num{0.65} & \num{0.74} & \num{0.50} & \num{0.71}\\
black\_p & \num{0.14} & \num{0.10} & \num{0.17} & \num{0.07} & \num{0.05} & \num{0.03} & \num{0.11} & \num{0.05}\\
\bottomrule
\end{tabular}
\end{table}

==> tables/nbh-summary-race.tex <==
\begin{table}
\centering
\begin{tabular}[t]{lrrrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{miami} & \multicolumn{2}{c}{new-york} & \multicolumn{2}{c}{phoenix} & \multicolumn{2}{c}{ } \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7}
\multicolumn{1}{c}{ } & \multicolumn{1}{c}{non-white} & \multicolumn{1}{c}{white} & \multicolumn{1}{c}{non-white} & \multicolumn{1}{c}{white} & \multicolumn{1}{c}{non-white} & \multicolumn{1}{c}{white} & \multicolumn{1}{c}{non-white} & \multicolumn{1}{c}{white} \\
\cmidrule(l{3pt}r{3pt}){2-2} \cmidrule(l{3pt}r{3pt}){3-3} \cmidrule(l{3pt}r{3pt}){4-4} \cmidrule(l{3pt}r{3pt}){5-5} \cmidrule(l{3pt}r{3pt}){6-6} \cmidrule(l{3pt}r{3pt}){7-7} \cmidrule(l{3pt}r{3pt}){8-8} \cmidrule(l{3pt}r{3pt}){9-9}
  & Mean & Mean  & Mean   & Mean    & Mean     & Mean      & Mean       & Mean       \\
\midrule
white\_p & \num{0.38} & \num{0.61} & \num{0.48} & \num{0.66} & \num{0.69} & \num{0.73} & \num{0.55} & \num{0.70}\\
black\_p & \num{0.12} & \num{0.11} & \num{0.11} & \num{0.08} & \num{0.05} & \num{0.03} & \num{0.08} & \num{0.05}\\
\bottomrule
\end{tabular}
\end{table}

==> tables/nbh-summary.tex <==
\begin{table}
\centering
\begin{tabular}[t]{lrrrrrrrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{4}{c}{miami} & \multicolumn{4}{c}{new-york} & \multicolumn{4}{c}{phoenix} & \multicolumn{4}{c}{ } \\
\cmidrule(l{3pt}r{3pt}){2-5} \cmidrule(l{3pt}r{3pt}){6-9} \cmidrule(l{3pt}r{3pt}){10-13}
  & Mean & Median & Min & Max & Mean & Median & Min & Max & Mean & Median & Min & Max & Mean & Median & Min & Max\\
\midrule
pop & \num{12082.80} & \num{3210.50} & \num{23.00} & \num{141988.00} & \num{32344.56} & \num{16735.50} & \num{48.00} & \num{344789.00} & \num{8798.35} & \num{2784.00} & \num{0.00} & \num{232488.00} & \num{13283.48} & \num{4029.00} & \num{0.00} & \num{344789.00}\\
sq.miles & \num{3.71} & \num{0.93} & \num{0.01} & \num{42.50} & \num{3.80} & \num{0.78} & \num{0.01} & \num{95.02} & \num{4.22} & \num{0.96} & \num{0.01} & \num{133.58} & \num{4.06} & \num{0.93} & \num{0.01} & \num{133.58}\\
dem\_p & \num{0.42} & \num{0.40} & \num{0.21} & \num{0.80} & \num{0.52} & \num{0.51} & \num{0.19} & \num{0.82} & \num{0.29} & \num{0.28} & \num{0.13} & \num{0.64} & \num{0.35} & \num{0.31} & \num{0.13} & \num{0.82}\\
rep\_p & \num{0.28} & \num{0.28} & \num{0.05} & \num{0.50} & \num{0.19} & \num{0.18} & \num{0.02} & \num{0.41} & \num{0.38} & \num{0.39} & \num{0.11} & \num{0.65} & \num{0.33} & \num{0.34} & \num{0.02} & \num{0.65}\\
white\_p & \num{0.55} & \num{0.57} & \num{0.01} & \num{0.98} & \num{0.62} & \num{0.69} & \num{0.01} & \num{0.97} & \num{0.73} & \num{0.75} & \num{0.15} & \num{1.00} & \num{0.68} & \num{0.73} & \num{0.01} & \num{1.00}\\
black\_p & \num{0.11} & \num{0.06} & \num{0.00} & \num{0.80} & \num{0.09} & \num{0.03} & \num{0.00} & \num{0.64} & \num{0.03} & \num{0.03} & \num{0.00} & \num{0.26} & \num{0.06} & \num{0.03} & \num{0.00} & \num{0.80}\\
\bottomrule
\end{tabular}
\end{table}

==> tables/survey-summary-full-sample-nycc.tex <==
\begin{table}
\centering
\begin{tabular}[t]{lrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{email} & \multicolumn{2}{c}{meta} & \multicolumn{2}{c}{ } \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5}
  & Mean & SD & Mean & SD & Mean & SD\\
\midrule
dem & \num{0.71} & \num{0.45} & \num{0.78} & \num{0.41} & \num{0.75} & \num{0.44}\\
rep & \num{0.20} & \num{0.40} & \num{0.11} & \num{0.32} & \num{0.16} & \num{0.36}\\
ericadams & \num{0.34} & \num{0.47} & \num{0.17} & \num{0.37} & \num{0.26} & \num{0.44}\\
age & \num{56.95} & \num{13.72} & \num{41.19} & \num{18.59} & \num{49.63} & \num{17.97}\\
female & \num{0.49} & \num{0.50} & \num{0.31} & \num{0.46} & \num{0.41} & \num{0.49}\\
white & \num{0.64} & \num{0.48} & \num{0.77} & \num{0.42} & \num{0.70} & \num{0.46}\\
income\_num & \num{114008.44} & \num{49553.43} & \num{103972.46} & \num{52130.09} & \num{109001.06} & \num{51075.79}\\
college & \num{0.48} & \num{0.50} & \num{0.41} & \num{0.49} & \num{0.44} & \num{0.50}\\
housing\_tenure & \num{16.10} & \num{8.71} & \num{9.00} & \num{9.42} & \num{12.82} & \num{9.71}\\
homeowner\_num & \num{0.50} & \num{0.50} & \num{0.27} & \num{0.44} & \num{0.39} & \num{0.49}\\
married & \num{0.50} & \num{0.50} & \num{0.32} & \num{0.47} & \num{0.42} & \num{0.49}\\
children\_home\_num & \num{0.37} & \num{0.48} & \num{0.19} & \num{0.39} & \num{0.28} & \num{0.45}\\
\bottomrule
\end{tabular}
\end{table}

==> tables/survey-summary-full-sample.tex <==
\begin{table}
\centering
\begin{tabular}[t]{lrrrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{miami} & \multicolumn{2}{c}{new-york} & \multicolumn{2}{c}{phoenix} & \multicolumn{2}{c}{ } \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7}
  & Mean & SD & Mean & SD & Mean & SD & Mean & SD\\
\midrule
dem & \num{0.48} & \num{0.50} & \num{0.57} & \num{0.49} & \num{0.38} & \num{0.49} & \num{0.44} & \num{0.50}\\
rep & \num{0.40} & \num{0.49} & \num{0.33} & \num{0.47} & \num{0.52} & \num{0.50} & \num{0.46} & \num{0.50}\\
biden & \num{0.57} & \num{0.50} & \num{0.65} & \num{0.48} & \num{0.49} & \num{0.50} & \num{0.53} & \num{0.50}\\
age & \num{61.78} & \num{14.16} & \num{60.13} & \num{13.37} & \num{64.11} & \num{12.98} & \num{62.89} & \num{13.41}\\
female & \num{0.44} & \num{0.50} & \num{0.45} & \num{0.50} & \num{0.48} & \num{0.50} & \num{0.46} & \num{0.50}\\
white & \num{0.65} & \num{0.48} & \num{0.72} & \num{0.45} & \num{0.86} & \num{0.34} & \num{0.79} & \num{0.41}\\
income\_num & \num{104906.32} & \num{49347.95} & \num{117303.44} & \num{48353.02} & \num{110876.69} & \num{48030.97} & \num{110913.65} & \num{48590.62}\\
college & \num{0.67} & \num{0.47} & \num{0.68} & \num{0.47} & \num{0.62} & \num{0.48} & \num{0.64} & \num{0.48}\\
housing\_tenure & \num{17.47} & \num{53.24} & \num{23.70} & \num{58.59} & \num{19.11} & \num{58.29} & \num{19.57} & \num{57.30}\\
homeowner\_num & \num{0.86} & \num{0.35} & \num{0.74} & \num{0.44} & \num{0.90} & \num{0.30} & \num{0.86} & \num{0.34}\\
married & \num{0.60} & \num{0.49} & \num{0.60} & \num{0.49} & \num{0.67} & \num{0.47} & \num{0.64} & \num{0.48}\\
children\_home\_num & \num{0.33} & \num{0.47} & \num{0.39} & \num{0.49} & \num{0.27} & \num{0.45} & \num{0.31} & \num{0.46}\\
\bottomrule
\end{tabular}
\end{table}

==> tables/survey-summary.tex <==
\begin{table}[h]
\centering
\footnotesize
\caption{Survey Sample Summary Statistics -- Control Sample}
\label{tab:surv-sum}
\begin{tabular}[t]{lrrrrrr|rr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Miami} & \multicolumn{2}{c}{NYC} & \multicolumn{2}{c}{Phoenix} & \multicolumn{2}{|c}{ Pooled} \\
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{(n = 474)} & \multicolumn{2}{c}{(n = 453)} & \multicolumn{2}{c}{(n = 1,600)} & \multicolumn{2}{|c}{(n = 2,527) } \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7}\cmidrule(l{3pt}r{3pt}){8-9}
  & Avg. & St. Dev. & Avg. & St. Dev. & Avg. & St. Dev.   & Avg. & St. Dev.   \\
\midrule
Democrat & \num{0.48} & \num{0.50} & \num{0.57} & \num{0.49} & \num{0.38} & \num{0.49} & \num{0.44} & \num{0.50} \\
Republican &\num{0.40} & \num{0.49} & \num{0.33} & \num{0.47} & \num{0.52} & \num{0.50} & \num{0.46} & \num{0.50} \\
Vote Biden 2020 &  \num{0.57} & \num{0.50} & \num{0.65} & \num{0.48} & \num{0.49} & \num{0.50} & \num{0.53} & \num{0.50} \\
Age & \num{61.78} & \num{14.16} & \num{60.13} & \num{13.37} & \num{64.11} & \num{12.98} & \num{62.89} & \num{13.41} \\
Female & 0.44 & 0.50 & 0.46 & 0.50 & 0.48 & 0.50 & 0.47 & 0.50 \\
White & 0.75 & 0.44 & 0.75 & 0.43 & 0.88 & 0.32 & 0.84 & 0.37\\
Income (1,000s) & 106.56 & 41.78 & 119.44 & 41.55 & 109.99 & 41.73 & 111.46 & 41.92 \\
College & 0.80 & 0.40 & 0.86 & 0.35 & 0.74 & 0.44 & 0.77 & 0.42 \\
Years Residence & 15.65 & 9.99 & 22.17 & 13.77 & 17.42 & 10.90 & 17.94 & 11.49 \\
Homeowner & 0.86 & 0.34 & 0.73 & 0.44 & 0.91 & 0.28 & 0.87 & 0.33 \\
Married & 0.65 & 0.48 & 0.59 & 0.49 & 0.68 & 0.47 & 0.66 & 0.47 \\
Children in Home & 0.35 & 0.48 & 0.38 & 0.49 & 0.29 & 0.45 & 0.32 & 0.47 \\
\bottomrule
\end{tabular}
\end{table}

